Hierarchical Adaptable and Transferable Networks (HATN) for Driving Behavior Prediction

When autonomous vehicles still struggle to solve challenging situations during on-road driving, humans have long mastered the essence of driving with efficient transferable and adaptable driving capability. By mimicking humans' cognition model and semantic understanding during driving, we present HATN, a hierarchical framework to generate high-quality driving behaviors in multi-agent dense-traffic environments. Our method hierarchically consists of a high-level intention identification and low-level action generation policy. With the semantic sub-task definition and generic state representation, the hierarchical framework is transferable across different driving scenarios. Besides, our model is also able to capture variations of driving behaviors among individuals and scenarios by an online adaptation module. We demonstrate our algorithms in the task of trajectory prediction for real traffic data at intersections and roundabouts, where we conducted extensive studies of the proposed method and demonstrated how our method outperformed other methods in terms of prediction accuracy and transferability.

==> 2related_works.tex <==
\section{Related works}
\subsection{Traditional methods}
The problem of predicting future motion for dynamic agents has been well studied in the literature. Classic physics-based methods include Intelligent Driver Model\cite{treiber2000congested}, Kalman Filter\cite{elnagar2001prediction}, Rapidly Exploring Random Trees\cite{aoude2010threat}, etc. These methods essentially analyze agents and propagate their historic and current state forward in time. Other classic pattern-based methods classify driving motion into semantically interpretable maneuver classes, via Hidden Markov Model\cite{deo2018would}, Gaussian Process\cite{9357407}, and Bayesian Network\cite{schreier2014bayesian}, which is then used to facilitate intention-and-maneuver-aware prediction. These methods have been performing well in scenarios with simple road geometry like highways, or sparse-interaction scenarios like calm streets. However, these methods struggle when confronting long-horizon prediction tasks or complex-road-geometry intense-interaction scenarios like crowded roundabouts and interactions. Such performance downgrade usually stems from the limited expressiveness of the model, insufficient interaction and context encoding, and laborious task-specific rule design. 
% Rule-based, struggles in the long horizon, especially in diverse maneuvers, limited by the expressiveness or complex rule design. 

\subsection{Deep-learning-based methods}
The success of deep learning ushered in a variety of data-driven methods. Due to the temporal nature of the prediction task, these models often embed Recurrent Neural Network (RNN) variants, such as LSTMs or GRUs, into the encoder-decoder architectures \cite{park2018sequence}\cite{hu2018framework}\cite{zyner2019naturalistic}. While these methods have shown great expressiveness with little human effort, the relationships among vehicles have been insufficiently reasoned. On the one hand, these methods are in lack of flexibility as they usually only consider a fixed number of agents. On the other hand, the same agents feed into the model with different order does not necessarily generates the same results. Such inconsistent results makes no sense as we are considering the same scene. To tackle these drawbacks, Graph Neural Network (GNN) has been recently combined with RNN in an explicit or implicit encoder decoder architecture for prediction tasks\cite{salzmann2020trajectron++}\cite{ding2019predicting}\cite{li2019grip++}\cite{ma2019trafficpredict}\cite{choi2019drogon}\cite{li2021hierarchical}\cite{hu2020scenario}. Due to the strong relational inductive bias of GNN\cite{battaglia2018relational}, these GNN-based methods successfully achieve flexibility in agent number and ordering invariance. Consequently, in this paper we also adopt a GNN-based architecture.
% RNN expressiveness. suffers in multi-agent systems, not only the variable number of agents, but also the interactions among agents.
% GNN, inductive biases. order invariant. 

\subsection{Hierarchical prediction}
Revisiting the driving task, there inherently exists a high-level intention determination sub-task and a low-level motion execution sub-task. Some GNN-based methods directly predict future motion in an end-to-end manner\cite{salzmann2020trajectron++}\cite{ma2019trafficpredict}\cite{li2019grip++}. However, such monolithic models are usually hard to learn, explain, and verify. To this point, some existing GNN-based methods exploit the hierarchies in the driving task\cite{ding2019predicting}\cite{choi2019drogon}\cite{li2021hierarchical}. These methods first generate the driving intention or pattern, and then conduct conditional trajectory prediction. However, though equipped with hierarchies, these methods are still trained in an end-to-end manner. Consequently, the two benefits of hierarchies, task simplification and representation filtering, are hardly exploited since the model is still monolithically used. In comparison, our method not only utilizes hierarchical design, but train the model hierarchically with the accessible ground-truth intention label. As a result, our method is not only able to monitor and refine the learning in each hierarchies, but will also enhance generalization since the resulting sub-policies take their own relevant features accordingly and can be easily plugged-and-reused in different tasks.

% still easily fail when transferred to similar or distinct scenarios after they are trained. The reasons can be two-fold: 1) These hierarchically designed methods are are still trained in an end-to-end manner. Consequently, the two benefits of hierarchies, task simplification and representation filtering, are hardly exploited as the the model is still monolithically used


% Ideally, such hierarchical designs will not only simplify the task by dividing it into several easier sub-tasks\citep{botvinick2009hierarchically}\cite{BerliacHierachialRL2019}, but also facilitate learning by selecting relevant features for each sub-tasks\cite{niv2019learning}\cite{radulescu2019holistic}. Typical hierarchical methods will result in several sub-policies which can be easily plugged-and-reused in different tasks\citep{bacon2017option}.

% Though more intepretable with more semantic, these methods tend to fail when they are transfered to a similar or distinct scenaiors

% These methods first generate an intention in the state space\cite{ding2019predicting}\cite{drogon}\cite{li2021hierarchical} or latent space\cite{tang2019multiple}
% \cite{tpnet}: end point, not graph
% \cite{rhinehart2019precog}: given goal, predict trajectory
% \cite{drogon}: divide image into 25 regions, goal in the image
% \cite{titan}: not graph, action recognition

% A Hierarchical Framework for Interactive Behaviour Prediction of Heterogeneous Traffic Participants Based on Graph Neural Network

% 2 tasks: passing order prediction or trajectory prediction. Passing order, requires further decoding. End-to-end monolithic methods output trajectories. Hard to learn, explain and verify. 

% Hierarchical methods. task simplification and representation filtering. latent space, state space. fail when transferred due to the absence of generic representation.

\subsection{Transferable prediction}
Ideally, we expect omni-potent prediction algorithms that can be applied to many different scenarios such as highways, intersections, and roundabouts. However, most existing methods either focus on certain scenarios\cite{ding2019predicting}\cite{choi2019drogon}, or train and apply their methods in various scenarios without assessing their scenario-wise performance\cite{salzmann2020trajectron++}\cite{ma2019trafficpredict}\cite{li2019grip++}\cite{li2021hierarchical}. As a result, these methods tend to fail when transferred to new different scenarios without learning a new set of model parameters. Looking deeper for reasons, the input features of these methods are either in Cartesian coordinate frame or scene images. The drawbacks of such design can be two-fold: 1) scenario-specific information such as traffic regulations and road geometries are hardly or only softly embedded. 2) these representations are not generic and will change each time a new scenario is encountered. 

Very few works have been addressing these limitations. One recent work\cite{hu2020scenario} achieves transferable prediction by designing generic representations called Semantic Graph, where Dynamic Insertion Areas rather than road entities are regarded as the nodes. In such representations, scenario-specific information such as road geometry and traffic regulations is hard-embed in a generic manner. However, this work only considers the high-level intention prediction sub-task and requires further motion decoding from the downstream module for practical use. In contrast, our paper adopt such generic representations and train the model hierarchically, which enable us to conduct intention prediction and motion prediction simultaneously.

% focuses on predicting vehicles' passing order in a transferable manner by designing scenario-generic representations. 

% generic representation, road geometry, traffic regulations;
% Transferability. trained end-to-end, Generic representation, not fail, transferable
% selecting interacting vehicles according to road geometry, traffic regulations.
% context info such as road geometry, traffic regulations.

\subsection{Adaptable prediction}
Apart from hierarchies and transferability, adaptability is another desired property of the prediction algorithms since there inevitably exists behavior variance in different individuals and scenarios. Consequently, online adaptation has been recently used in the human prediction research field. \cite{cheng2019human}\cite{8814238}\cite{cheng2020towards} adopts recursive least sqaure parameter adaptation algorithm (RLS-PAA) to adapt the parameter of the last layer in the neural network. To be able to conduct multi-step adaptation on random sets of parameters, \cite{abuduweili2021robust}\cite{9281312}\cite{abuduweili2020robust} utilizes modified extended kalman filter (MEKF$_{\lambda}$) to conduct model linearization and empirically compares the results of adapting different sets of parameters with different steps. The recent work most related to ours\cite{abuduweili2021robust}  adopts an encoder-decoder architecture for multi-task prediction, namely tasks of intention and trajectory prediction. However, compared to our method, the benefit of GNN, hierarchical training, and transferable generic representation is not considered.

% However, these methods only adopt either DNN\cite{cheng2019human}\cite{cheng2020towards} or RNN\cite{abuduweili2021robust}\cite{9281312}\cite{abuduweili2020robust}\cite{8814238}, while GNN is not considered for better relationship reasoning.



% Compared to the most related and recent approach\cite{abuduweili2021robust}, we 

% AGen: Adaptable Generative Prediction Networks for Autonomous Driving
 
% Human Motion Prediction using Semi-adaptable Neural Networks 

% Adaptable Human Intention and Trajectory Prediction for Human-Robot Collaboration

% Robust nonlinear adaptation algorithms for multitask prediction networks

% Adaptation. all parameter. trajectory prediction. 






==> 4high_level_policy0.tex <==
% \begin{figure*}[t]
%     \centering
%     \includegraphics[width=0.9\textwidth]{Figures/Architecture.pdf}
%     \caption{The proposed method consists of 4 parts: 1) As on the left, for one selected ego car, we first extract its interacting vehicles and generate all the dynamic insertion areas (DIA) which the ego vehicle can choose to insert into. The DIAs are then used as nodes to construct a semantic graph (SG). 2) Taking SG as input, the high-level Semantic Graph Network (SGN) is responsible for reasoning relationships among vehicles and output intention signals, such as which area to insert into and corresponding goal position. 3) The low-level Encoder Decoder Network (EDN) takes each vehicle's historic dynamics and intention signal, and predicts their future trajectory. 4) The Online Adaptation module can online adapt EDN's parameter based on historic prediction errors, to capture individual-and-scenario-specific behaviors.}
%     \vspace{-2em}
%     \label{fig:architecture}
% \end{figure*}
\section{High-level intention-identification policy}
\label{appendix:SGN}
In this section, we first
adopt the semantic graph (SG), where the dynamic insertion area (DIA) is
defined as a generic and compact representation of the scenario. We then introduce the semantic graph network
(SGN) which generates agents' intention by reasoning about their internal relationships. The advantages of introducing dynamic insertion
area can be threefold: (1) It explicitly describes humans' insertion behavior considering map, traffic regulations, and interaction information. (2) It filters scene information and only extracts a compact set of vehicles and states crucial for the intention identification. (3) DIA is a generic representation, which can be used across different scenarios. 

\subsection{Semantic graph}
Initially introduced in \cite{hu2020scenario}, the semantic graph (SG) is a generic spatial-temporal representation of the environment. Specifically, SG utilize Dynamic Insertion area as basic nodes, which is 

\subsubsection{Static information}
The static information is extracted from the scene to describe road geometries, traffic regulations and their inter-connections. Specifically, we distill all the static information into road references paths, which can be obtained from the HD map or by averaging human driving paths from collected data. As in Figure~\ref{fig:semantic graph} The topological relationships among references (reference path crossing) is represented by the conflict point or merge point on the paths. The traffic regulations (stop sign, yield sign, etc.) is reflected by break points on the reference path. Such a reference-based representation naturally calls for Frenet coordinate to be utilized through out this paper.

Mathematically, each road reference path is defined as a series of way points on a polynomial curve, namely ${\mathcal{X}}_{ref} = \{(x_k, y_k),...\}$, where $x$ and $y$ denote location of each point, and $k$ denotes the k-th point. The conflict point is the reference point closest to the crossing reference path and denoted as $(x, y)^c$. The merge point is the denoted as $(x, y)^m$ while the break point divides long road paths into several segments with different traffic regulations and $(x, y)^b$.  

\subsubsection{Dynamic information}
For the dynamic information, we utilize the Dynamic Insertion Area  (DIA)\cite{hu2020scenario}\cite{hu2018probabilistic} as a semantic and generic representation. The dynamic insertion area is semantically defined as: \textit{a dynamic area that can be inserted or entered by agents on the roads.} As illustrated in Figure~\ref{fig:semantic graph}, a dynamic insertion area is constructed by four boundaries. The front or rear boundary are formulated by road entities\footnote{The DIA boundaries can be formulated by any types of road entities including vehicles, cyclists and pedestrians. However, in this work, we will focus on vehicles only.} or points on the reference. When the merge point, conflict point and break point is used as a bound of the DIA, the relationships among reference line and traffic regulation information are naturally incorporated into the DIA. Considering that the side boundaries are formulated by connecting the front and rear boundary along the road or curbs, the road geometry information is also naturally entailed in the shape of the area. 

\begin{figure}[t]
    \centering
    \includegraphics[width=0.35\textwidth]{Figures/DIA.pdf}
    \caption{Illustration for reference line, critical reference points, and formulation of dynamic insertion area.}
    % \vspace{-2em}
    \label{fig:semantic graph}
\end{figure}

Mathematically, we define each dynamic insertion area as $\mathcal{A} = (\mathcal{X}_f, \mathcal{X}_r, \mathcal{X}_{ref})$. $\mathcal{X}_{f/r} = (x_{f/r}, y_{f/r}, v_{f/r}, \theta_{f/r} )$ denotes the properties for the center point of front bound and rear boundary of the DIA (location, velocity and orientation); $\mathcal{X}_{ref}$ denotes the information of the reference path that the area is currently on, where the property of side boundary is also explicitly incorporated. 

\subsubsection{DIA extraction}
\label{Sec:DIA Extraction}
With these definitions, we then need to decide which DIAs worth consideration in a scene. Many existing methods\cite{salzmann2020trajectron++}\cite{park2018sequence}\cite{li2019grip++} select interacting vehicles according to distance criteria. However, we argue that distance may not sufficiently or necessarily determine interaction. For instance, close vehicles that are running on the opposite-direction lane may hardly be intervening with each other. Instead, interactions essentially happen among vehicles which are driving into a common area. Thus we choose the vehicles whose reference paths intersect with ego vehicle's reference path as the interacting vehicles. The DIAs are then generated only for these interacting vehicles. Note such a selection procedure can effectively help to focus our attention and computation resources on critical vehicles and ignore unrelevant vehicles. 

To capture each DIA's crucial information for humans' insertion decision, we further extract three high-level features under the Frenet coordinate: $d_{f/r}^{lon}$ denotes longitudinal distance to active conflict point $rpt_{act}$ of front or rear boundary. $l = d_r^{lon} - d_f^{lon}$ measures the length of the DIA. To facilitate relationship inference among DIAs, we also define the relative feature for each DIA by aligning it with the reference DIA. Note that we choose front DIA as the reference DIA because the ego vehicle is implicitly represented by the rear boundary of the front DIA. For more detailed description on the DIA properties, DIA extraction algorithm, and feature selection, one can refer to \cite{hu2020scenario}\cite{hu2018probabilistic}.

\subsubsection{Semantic graph construction}
With the extracted DIAs, we can construct a 3D spatial-temporal semantic graph
${\mathcal{G}^{t\rightarrow t^{'} }} = ({\mathcal{N}^{t\rightarrow t^{'} }}, {\mathcal{E}^{t\rightarrow t^{'} }})$, 
where $t\rightarrow t{'}$ denotes the time span from a time step $t$ to time step $t'$ with $t{'}>t$. Node $n_i^{t_i} \in {\mathcal{N}^{t\rightarrow t^{'} }} $ represents the $i$th DIA at time step $t_i$, which is associated with an absolute feature vector $x_i^{t_i}$ and a relative feature vector $x{'}_i^{t_i}$.  Edge $e_{ij}^{t_i \rightarrow t_j} = (n_i^{t_i}, n_j^{t_j})$ denotes the directed edge from node $n_i$ at time step $t_i$ to node $n_j$ at time step $t_j$, which is associated with feature vector $x_{ij}^{t_i \rightarrow t_j}$. Note that the graph is also flexible to describe variable number of agent as time evolves.

Compared to formulating individual entities as the nodes in most graph-based methods\cite{li2019grip++}\cite{salzmann2020trajectron++}\cite{li2020evolvegraph}, we instead utilize DIAs. On the one hand, the representation of DIA still only allows us to describe vehicles' dynamics and interaction as any vehicle' information is covered by the DIA in front of it. On the other hand, the map and regulation information are naturally and generically incorporated into the semantic graph without extra effort of encoding. Consequently, the elicitation of DIA offers a more semantic and compact scene understanding of various driving situations, mitigating policy's learning burden. For instance, when the ego vehicle's policy decides to insert into a DIA, it is simultaneously passing the rear-boundary vehicle and yielding the front-boundary vehicle as in Figure~\ref{fig: one insertion}(a). 

\subsection{Semantic graph network}
As the high-level intention identification policy, the architecture of the SGN is shown in Figure \ref{fig:architecture}. SGN takes the spatial-temporal 3D semantic graph from historic time step $t-T_h$ to current time step $t$ as the input, rather than only spatial 2D semantic graph of current time step $t$\cite{hu2020scenario}. Such change aims at capturing more temporal dynamics and interactions among vehicles. SGN then decides which area to insert into and generate the associated goal state distribution. The mean of the goal state distribution is then delivered to low-level policy for generating more human-like behaviors especially in the long term. 

\subsubsection{Feature encoding layer}
In this layer, we essentially encode the sequence of absolute and relative node features mentioned in Sec.\ref{Sec:DIA Extraction} from historic time step $t-T_h$ to current time step $k$ recursively:
\begin{equation}
	h^t_i = f^1_{rec}(\textbf{X}^t_i)
\end{equation}
\begin{equation}
	h{'}^t_i = f^2_{rec}(\textbf{X}{'}^t_i)
\end{equation}
where $\textbf{X}^t_i=[x^{t-T_h}_i, ..., x^{t}_i]$ and  $\textbf{X}{'}^t_i=[x{'}^{t-T_h}_i, ..., x{'}^{t}_i]$ respectively denotes the absolute feature and relative feature of node $i$ from time step $t-T_f$ to current time $t$; $h^t_i$ and $h{'}^t_i$ denote the hidden states encoded from absolute and relative features respectively, also the outputs of the recurrent function $f^1_{rec}$ and $f^2_{rec}$\footnote{We choose graph recurrent unit (GRU) as our recurrent function for the iterative encoding process.}; $h^{t-1}_i$ and $h{'}^{t-1}_i$ denote the previous hidden state.

\subsubsection{Relationship reasoning layer}
\label{sec:Relationship Reasoning Layer}
To infer relationships between any two nodes, we firstly embed the hidden state encoded from the relative feature from last layer:
\begin{equation}
	\hat{h}{'}^t_i = f^1_{enc}(h{'}^t_i)
\end{equation}
 We secondly exploit soft-attention mechanism\cite{velivckovic2017graph}\cite{luong2015effective}\cite{bahdanau2014neural} to compute the node $n_i$'s attention coefficients on node $n_j$:
\begin{equation}
	a^t_{ji} = f_{att}(concat(\hat{h}{'}^t_j, \hat{h}{'}^t_i); \textbf{W}_{att})
\end{equation} 
where function $f_{att}$ maps each concatenated two features into a scalar, parameterized by $\textbf{W}_{att}$. The attention coefficient is then normalized across all nodes $\mathcal{N}^t$ at time step $t$:
\begin{equation}
	\alpha^t_{ji} = \frac{exp(a^t_{ji})}{\sum_{n\in \mathcal{N}^t}exp(a^t_{ni})}
\end{equation}
Eventually, node $n_i$'s relationships with all nodes is derived by the attention-weighted summation of all encoded relative features\footnote{The attention-based relationship reasoning is conducted for all nodes.}:
\begin{equation}
	\bar{h}^t_i = \sum_{n\in \mathcal{N}^t} \alpha^t_{ni} \odot \hat{h}{'}^{t}_{n}
\end{equation} 
where $\odot$ denote element-wise multiplication.


\subsubsection{Intention generation layer}
When deciding which area to insert into, not only the node relationships are needed, but also each node's own features are required. Thus we first concatenate and encode each node's embedded absolute and relative feature:   
\begin{equation}
	\widetilde{h}^t_i =  f^2_{enc}(concat(\hat{h}^t_i, 	\hat{h}{'}^t_i))
\end{equation}
Each DIA's future evolution in the latent space is then derived by combining encoded node relationships and features:
\begin{equation}
	z_i^t = f^3_{enc}(concat(\bar{h}^t_i, \widetilde{h}^t_i))
\end{equation} 
The latent vector of each DIA is then used to generate the probability of being inserted by ego vehicle: 
\begin{equation}
	\label{eq:insert_probability}
	w_i^t = \frac{1}{1 + exp(f^1_{out}(z_i^t))}
\end{equation} 
which is then normalized across all DIAs in current time step such that $\sum_{i \in \mathcal{N}^t}w_i^t = 1$.
Moreover, to generate a practical intention signal for low-level policy to leverage, we further use Gaussian Mixture Model (GMM) to generate probabilistic distribution of each DIA's future goal state $g$ in a certain horizon\footnote{In this paper, we use the relative traveled distance in future 3 seconds as the goal state representation, encoded by historic information in last 1 second}:
\begin{equation}
	f(g_i^t|z_i^t) = f(g_i^t|f^2_{out}(z_i^t))
\end{equation}
where the function $f^2_{out}$ maps the latent state $z_i^t$ to the parameters of GMM (i.e. mixing coefficient $\alpha$, mean $\mu$, and covariance $\sigma$). 

\subsubsection{Loss function}
We not only expect the largest probability to be associated with the actual inserted area ($\mathcal{L}_{class}$), but also the ground-truth goal state to achieve the highest probability in the output distribution ($\mathcal{L}_{regress}$). Thus we define the loss function as:
\begin{equation}
\begin{split}
	\mathcal{L} &= \mathcal{L}_{regress} +\beta \mathcal{L}_{class}\\
				&= - \sum_{\mathcal{G}_s} \bigg(\sum_{i \in \mathcal{N}^s}log\Big(   p\big(\check{g}_i|f^2_{out}(z_i)\big)\Big)+\beta \sum_{i \in \mathcal{N}^s} \check{w}_i log(w_i)\bigg)
\end{split}
\end{equation}
where $\mathcal{G}_s$ denotes all the training graph samples; $\mathcal{N}^s$ denotes all the nodes in one training graph sample; $\check{y}_i$ and $\check{w}_i$ denotes the ground-truth label for goal state and insertion probability of node $n_i$. We output the goal state for all interacting vehicles rather than ego vehicle exclusively\cite{hu2020scenario} to encourage sufficient relationship and interaction reasoning, and also realize data augmentation. 

Also note that though not directly used by low-level behavior-generation policy, the insertion probability learning still serving as an auxiliary task to stabilize main-stream goal state learning\cite{mirowski2016learning}\cite{hasenclever2020comic}. Defining goal state in the state space instead of the latent space also offers us accessible labels to monitor the high-level policy learning alone. The detailed introduction of the layer can be found in Table~\ref{tab:GNN table} of the appendix.


==> 7experiment0.tex <==
\section{Experiment}
In this section, we evaluate the capability of the proposed algorithm in different aspects, where the performance of sub-policies, overall performance, transferability, and adaptability are examined. 
\subsection{Experiment Setting}
We verified our proposed method with real human driving data from the INTERACTION dataset\cite{interactiondataset}. Two different scenarios are utilized as in Figure~\ref{fig:sequence of insertion} and Figure~\ref{fig:transferability}: a 5-way unsignalized intersection and an 8-way roundabout. All vehicle data are collected by a drone from bird-eye view with 10 Hz sampling frequency. Road reference paths and traffic regulations are extracted from the provided high-definition map. 

The intersection scenario is used to train our policy and evaluate the performance of behavior prediction. The roundabout scenario is used to evaluate the transferability of our method. In the intersection scenario, we have 19084 data points, which are split to 80\% of training data and 20 \% of testing data. In the roundabout scenario, we have 9711 data points to evaluate transferability.

In our experiments, we choose the historic time steps $T_h$ as 10 and future time step $T_f$ as 30 steps, which means we utilize historic information in past 1 seconds to generate future behavior in next 3 seconds. In addition to the long-term behavior prediction evaluation in the whole future 30 steps, we also evaluated short-term behavior prediction in the future 3 steps in Sec \ref{sec:overall_evaluation}, as short-term behavior is safety-critical especially in close-distance interactions.

The method was implemented in Pytorch on a desktop computer with an Intel Core i7 9th Gen CPU and a NVIDIA RTX 2060 GPU. For each model, We performed optimizations with Adam and sweep over more then 20 combinations of hyperparameter to select the best one including batch size, hidden dimension, learning rate, dropout rate. For each combination of hyperparameter, we trained 1000 epochs for the SGN and EDN respectively.

\subsection{Case Study}
We first show how our method works with 3 examples. 
\subsubsection{One Insertion Process} As in Figure~\ref{fig: one insertion}, we first show how our method works in one insertion process. Once we choose the ego vehicle, its interacting vehicles and corresponding DIAs are extracted. Our method would then predict the intention and future trajectory of the ego vehicle and its interacting vehicles. 

In the figure, we drew the ego vehicle with white color, the interacting vehicles with bright colors, and the non-interacting vehicles with transparent colors. The darker one DIA is, the more likely the ego vehicle would insert into that DIA. The future trajectories of ego vehicle and interacting vehicles are also displayed with the corresponding color.

As in Figure~\ref{fig: one insertion}(a)(b), we can see that at the very beginning, the white ego car had 5 areas to choose to insert into: $A_1, A_2, A_3, A_4, A_5$. At this time, ego vehicle braked so our method predicted that it would insert into its front DIA $A_1$, which means yielding to other vehicles. In the Figure~\ref{fig: one insertion}(c), the blue vehicle behind DIA $A_3$ passed away and the ego vehicle accelerated, so our method predicted ego vehicle would insert into DIA $A_2$, which means passing before other vehicles. In Figure~\ref{fig: one insertion} (d) we can see the ego vehicle crossed the conflict area and finished this insertion.

\subsubsection{A Sequence of Insertion Processes} In Figure~\ref{fig:sequence of insertion}, we show how one vehicle crossed the intersection with a sequence of insertion processes. 

In Figure~\ref{fig:sequence of insertion}(a), the ego vehicle initially interacted with the upper red vehicle. As the white ego vehicle was running in a high speed, our method predicted it would insert into DIA $A_2$, which means passing the red vehicle. After finishing the first insertion, in Figure~\ref{fig:sequence of insertion}(b) the ego vehicle then interacted with the yellow vehicle below. Our method predicted the ego vehicle would continue to pass and insert into the DIA $A_3$.

Next, in Figure~\ref{fig:sequence of insertion}(c), the ego vehicle's path conflicted with that of the purple and green car. The ego vehicle first decelerated and our method predicted it would insert into its front DIA $A_1$ and yield other cars. In Figure~\ref{fig:sequence of insertion}(d), after the purple car passed away, the ego vehicle then accelerated and inserted into DIA $A_5$ to pass ahead of the green car.

\subsubsection{Scenario-Transferable Insertion Process} In Figure~\ref{fig:transferability}, we show that after our method is trained in the intersection scenario, it can be zero-transferred to the roundabout scenario.

In Figure~\ref{fig:transferability}(a), the ego vehicle just entered the roundabout with some speed, so it was equally likely to insert into the three DIAs $A_1, A_2, A_3$. In Figure~\ref{fig:transferability}(b), the ego vehicle decelerated, which means that it would yield other vehicles and insert into its front DAI $A_1$. 

In Figure~\ref{fig:transferability}(c), the green car passed away but the ego vehicle still remained a low speed, leading to the prediction that it would continue to yield. Nevertheless in Figure~\ref{fig:transferability}(d), the ego vehicle accelerated so it became equally likely to insert into either DIA $A_1$ or DIA $A_3$. In Figure~\ref{fig:transferability}(e) the ego vehicle gained a high speed, and thus our method predict it would pass before the purple car by inserting into DIA $A_3$. 

After finishing the insertion in Figure~\ref{fig:transferability}(f),  the ego vehicle continued to run while there were no other vehicles interacting as in Figure~\ref{fig:transferability}(g). In Figure~\ref{fig:transferability}(h), one green car entered the roundabout and the ego vehicle decided to pass before it by inserting into DIA $A_4$.

\subsection{Semantic Graph Network Evaluation}
\begin{figure*}[t]
    \centering
    \includegraphics[width=0.95\textwidth]{Figures/intersection1.pdf}
    \caption{Case Study - One insertion process. White car denotes the ego car; Bright-color cars denote ego car's interacting vehicles and DIAs are extracted for them. The darker one DIA is, the more likely ego car is going to insert into that area. As in (a)(b), ego car has 5 DIAs to insert into $A_1, A_2, A_3, A_4, A_5$. As ego car is in low speed, our method predicts it would insert into its front DIA and yield other vehicles. In (c), the blue car passes away and the ego vehicle accelerates. So our method predict it would insert into $A_2$ and pass before other vehicles. In (d), the ego vehicle crossed the conflict area and finished one insertion process.}
    \label{fig: one insertion}
    % \vspace{-2em}
\end{figure*}

\begin{figure*}[t]
    \centering
    \includegraphics[width=0.95\textwidth]{Figures/intersection2.pdf}
    \caption{Case Study - A sequence of insertion processes. In (a), ego car firstly interact with the red car and decided to insert into DIA $A_2$ and pass before the red car. In (b), after the first insertion, ego car interacts with the yellow car and decides to continue pass it by inserting into $A_3$. In (c), ego vehicle then interact with the purple and green vehicles and decides to insert into its front DIA and yield other cars. In (d), the purple car passes way, so the ego car accelerates to insert into DIA $A_5$ and pass the green car.}
    \label{fig:sequence of insertion}
    % \vspace{-1em}
\end{figure*}

\begin{figure*}[t]
    \centering
    \includegraphics[width=0.95\textwidth]{Figures/roundabout.pdf}
    \caption{Case Study - Insertion behavior transfered to the roundabout scenario: Trained in the intersection scenario, our method can be directly transferred to the roundabout scenario. In (a), when the white ego vehicle enters the roundabout, it has some speed and is equally likely to insert into the three DIA $A_1, A_2, A_3$. In (b), ego vehicle decelerates and decides to insert into its front DIA, yielding other vehicles. In (c), the green car passes but the ego vehicle remains in a low speed, so our method predict it would continue to yield the purple car. In (d), the ego vehicle accelerates, so it becomes equally possible in passing and yielding. In (e), the ego vehicle gains a high speed and decides to insert into $A_3$ to pass the purple car. In (f), the ego vehicle finishes the insertion. In (g), the ego vehicle continues to run, and at that time there is not other interacting vehicles. In (h), the green car enters the roundabout, and the ego car decides to insert into $A_4$ to pass before the green car.}
    \label{fig:transferability}
    % \vspace{-1em}
\end{figure*}



\begin{table*}[t]
		\centering
		\begin{tabular}{cc|ccc|cccc} 
			\toprule 
			& & \multicolumn{3}{c|}{Representation Ablation Study} & \multicolumn{4}{c}{Architecture Ablation Study}\\
			\midrule 
			Scenario & Measure & No-Temporal & GAT & Single-Agent & Two-Layer-Graph & Multi-Head & Seq-Graph & Ours\\
			\midrule 
			\multirow{2}*{Intersection} &  Prob (\%) & 87.44 ± 33.13 & \textbf{91.93 ± 27.05} & 88.8 ± 31.53 & 90.15 ± 29.79 & 90.00 ± 30.00 & 89.8 ± 30.24 & 90.50 ± 28.70\\
			~ & ADE (m) & 1.59 ± 1.67 & 1.18 ± 1.51 & 1.04 ± 0.90 & 0.98 ± 0.93 & 0.97 ± 0.75 & 1.33 ± 1.91 & \textbf{0.94 ± 0.73}\\
			\midrule    
			
			\multirow{2}*{\tabincell{c}{Roundabout\\(Transfer)}} &  Prob (\%) & \textbf{93.92 ± 23.88} & 91.21 ± 28.12 & 92.20 ± 26.75 & 90.54 ± 29.26 & 92.10 ± 26.96 & 91.60 ± 27.62 & 90.70 ± 29.08\\
			~ & ADE (m) & 3.62 ± 6.72 & 2.70 ± 5.16 & 1.88 ± 2.48 & 1.87 ± 2.51 & 2.79 ± 20.78 & 3.10 ± 3.10 & \textbf{1.70 ± 1.99}\\
			\bottomrule 
		\end{tabular} 
		\caption{The quantitative results for high-level intention identification polices.} 
		\label{tab:graph}
		
		
		\vspace{-2em}
\end{table*}

In the high-level intention-identification task, we compared the performance of our semantic graph network (SGN)  with that of other six approaches. Three of them are exploring the effect of different representation in the input and output. And the rest of them are the variations of the proposed network for ablation study, which explored the effect of frequently used network architectures and tricks.

\begin{enumerate}
    \item No-Temporal: This method does not take historic information into account, namely only consider the information of current time step $t$.
    \item GAT: This method use absolute feature to calculate relationships among nodes, and no relative feature is defined, which corresponds to the original graph attention network\cite{velivckovic2017graph}.
    \item Single-Agent: This method only considers the loss of ego vehicle in each graph training sample.
    \item Two-Layer-Graph: This method has two-layer graph to conduct information embedding, namely exploits aggregation twice\cite{sanchez2018graph}.
    \item Multi-Head: This method employs the multi-head mechanism, expecting to stabilize learning\cite{velivckovic2017graph}. This method operates the relationship reasoning in Sec.\ref{sec:Relationship Reasoning Layer} multiple times in parallel independently, and concatenate all aggregated features as the final aggregated feature. In our case, we set the head number as 3.  
    \item Seq-Graph: This methods first conducts relationship reasoning for the graph at each time step and second feeds the sequence of aggregated graphs into RNN for temporal processing. As a comparison, our method first embeds each node's sequence of historic features with RNN and second conduct relationship reasoning using each node's hidden state from RNN at current time. 
\end{enumerate}

The models were trained and tested on the intersection scenario. The trained models were also directly tested on the roundabout scenario, which aimed at evaluating the zero-shot transferability. The performance of insertion identification was evaluated by calculating the multi-class classification accuracy. The performance of goal state generation was evaluated by the absolute-distance-error (ADE) between the generated goal state and ground-truth state.

According to the result shown in Table~\ref{tab:graph}, we can see for the \textbf{insertion identification task}, one big view is that all models achieved close accuracy of around 90\%, generally benefit from our representation of semantic graph. Another big view is that most models' transferability performance in the roundabout scenario surprisingly surpassed the performance in the intersection scenario which the models were originally trained. This is basically because intersection is a harder scenario than roundabout, as the vehicles need to interact with many vehicles from different directions simultaneously when they are entering the intersection, while vehicles in the roundabout only need to interact with the cars either from nearby branches or in close distance.

By a detailed analysis for insertion accuracy, though the model's performance were close, the GAT had the highest performance while our method followed as the second. The No-Temporal method had the lowest accuracy and largest variance in intersection scenario (87.44±22.13\%). This is because it is lacking in the temporal information, which can efficiently help to identify which DIA to insert into by introducing historic speed and acceleration. What is interesting is that the No-Temporal method contrarily achieved the highest insertion accuracy (93.92±23.88) in the roundabout scenario. One possible explanation is that the absence of temporal information constrained the model's capability and thus avoided over-specification, so the No-Temporal method has the best transferability performance. Such guess also helps to explain why the Two-Layer-Graph method had the lowest insertion accuracy in the roundabout scenario (90.54±29.26\%), as twice aggregations makes the model brittle to over-specification. 

The \textbf{goal state generation task}, on the one hand, is practically more important as it is directly delivered to low-level policy to guide the behavior generation process. On the other hand, it is much harder than the insertion identification task as it requires more delicate information extraction and inference. Consequently, we can see that the performance of different models varied a lot. Also, the models' performance significantly down-graded when they were directly transferred to the roundabout scenario, as the two scenarios have different geometries and different driving patterns such as speed and steering. 

Specifically, our method achieved the lowest error in both intersection and roundabout scenarios, while the No-Temporal method was the worst in both intersection and roundabout scenario, due to the lack of temporal information. As a comparison, the GAT method reached higher errors than ours method especially in the roundabout scenario, which shows the necessity of the relative features as it might be helpful for better inference and distribution shift resistance. Our method outperformed the Single-Agent method, which implies the advantages of data augmentation and encouraging interaction inference by taking all vehicles' generated goal state into the loss function. The Two-Layer-Graph method 
was the closest one to our method, while it came with serious over-fitting according to our training log. The Multi-Head method achieved the second best accuracy in intersection scenario but much worse performance in roundabout scenario, which might require more careful tuning or searching for a proper head number. The Seq-Graph method was the second worst in both the intersection and the roundabout scenario, which may imply that the complex encoding for past interactions could hardly help learning but indeed makes the learning harder. 


% \subsection{Low-Level Behavior Generation Policy Evaluation}
% We incrementally analyzed the performance of EDN, by first explore the performance of encoder decoder itself without intention signal and the performance of encoder decoder with intention signal. Such analysis aims at providing instructional experience on how to employ sequence-to-sequence model to the application of autonomous driving.  


\begin{table}[!t]
		\centering
		\begin{tabular}{c|cc|cc} 
			\toprule 
            \multirow{2}*{\tabincell{c}{(a)\\Coordinate\\Study}} &
			\multicolumn{2}{c|}{Intersection} & \multicolumn{2}{c}{Roundabout (Transfer)}\\
			
			\cmidrule(r){2-5} 
			~ & ADE & FDE & ADE & FDE\\
			\midrule 
			Cartesian & 1.53 ± 1.22 & 2.90 ± 2.77 & 12.57 ± 5.68 & 19.77 ± 7.43 \\
			\textcolor{red}{Frenet} & \textbf{0.91 ± 0.59}
            & \textbf{1.87 ± 1.48} & \textbf{2.96 ± 4.65} & \textbf{5.52 ± 7.20} \\
			
			
			\midrule 
			\bottomrule 
		\end{tabular} 
		\vspace{1em}
		
		
		\begin{tabular}{cc|cc|cc} 
			\toprule 
			\multicolumn{2}{c|}{\tabincell{c}{(b) Speed\\Ablation}} &
			\multicolumn{2}{c|}{Intersection} & \multicolumn{2}{c}{Roundabout (Transfer)}\\
			
			\midrule 
			\tabincell{c}{In} &\tabincell{c}{Out}
			&ADE & FDE & ADE & FDE\\
			\midrule 
			× & × & 0.91 ± 0.59 & 1.87 ± 1.48 & 2.96 ± 4.65 & 5.52 ± 7.20 \\
			\textcolor{red}{\checkmark} & \textcolor{red}{×} & 0.71 ± 0.54
            & 1.53 ± 1.27 & \textbf{2.33 ± 3.84} & \textbf{4.30 ± 5.44} \\
			× & \checkmark & 0.78 ± 0.53 & 1.74 ± 1.41 & 2.51 ± 4.16 & 4.97 ± 6.35 \\
			\checkmark & \checkmark & \textbf{0.70 ± 0.49} & \textbf{1.46 ± 1.26} & 2.40 ± 4.10 & 4.67 ± 6.03 \\
			
			\midrule 
			\bottomrule 
		\end{tabular} 
		\vspace{1em}
		
		\begin{tabular}{cc|cc|cc} 
			\toprule 
			\multicolumn{2}{c|}{\tabincell{c}{(c) Yaw\\Ablation}} &
			\multicolumn{2}{c|}{Intersection} & \multicolumn{2}{c}{Roundabout (Transfer)}\\
			
			\midrule 
			\tabincell{c}{In} &\tabincell{c}{Out}
			&ADE & FDE & ADE & FDE\\
			\midrule 
			× & × & 0.71 ± 0.54 & 1.53 ± 1.27 & 2.33 ± 3.84 & 4.30 ± 5.44 \\
			\textcolor{red}{\checkmark} & \textcolor{red}{×} & \textbf{0.67 ± 0.46} & \textbf{1.45 ± 1.19} & \textbf{2.23 ± 3.95} & \textbf{4.14 ± 5.19} \\
			× & \checkmark & 0.73 ± 0.50 & 1.59 ± 1.36 & 2.34 ± 3.96 & 4.49 ± 6.46 \\
			\checkmark & \checkmark & 0.67 ± 0.48 & 1.46 ± 1.24 & 2.51 ± 4.60 & 4.77 ± 6.43 \\
			
			\midrule 
			\bottomrule 
		\end{tabular} 
		\vspace{1em}
		
				
% 			\midrule 
% 			\checkmark & × & \checkmark & × & \checkmark & × & × & × & 0.48 ± 0.44 & 1.32 ± 1.32 & 1.26 ± 0.95 & 3.04 ± 2.44  \\
% 			\checkmark & × & \checkmark & × & × & \checkmark & × & × & 0.43 ± 0.35 & 1.36 ± 1.19 & 1.07 ± 1.10 & 2.66 ± 2.31 \\
% 			\checkmark & × & \checkmark & × & \checkmark & \checkmark & × & × & 0.41 ± 0.33 & 1.29 ± 1.14 & 0.96 ± 0.80 & 2.53 ± 2.13 \\
			
% 			\midrule 
% 			\checkmark & × & \checkmark & × & \checkmark & \checkmark & \checkmark & × & 0.41 ± 0.34 & 1.32 ± 1.16 & 0.97 ± 0.83 & 2.54 ± 2.14 \\
% 			\checkmark & × & \checkmark & × & \checkmark & \checkmark & × & \checkmark & 0.43 ± 0.34 & 1.32 ± 1.13 & 1.10 ± 1.32 & 2.57 ± 2.50 \\
		
		\begin{tabular}{cc|cc|cc} 
			\toprule 
			\multicolumn{2}{c|}{\tabincell{c}{(d) Repre\\Ablation}} &
			\multicolumn{2}{c|}{Intersection} & \multicolumn{2}{c}{Roundabout (Transfer)}\\
			
			\midrule 
			\tabincell{c}{Inc} &\tabincell{c}{Ali}
			&ADE & FDE & ADE & FDE\\
			\midrule 
			× & × & 0.67 ± 0.46 & 1.45 ± 1.19 & 2.23 ± 3.95 & 4.14 ± 5.19 \\
			× & \checkmark & 0.48 ± 0.44 & 1.32 ± 1.32 & 1.26 ± 0.95 & 3.04 ± 2.44 \\
			\checkmark & × & 0.43 ± 0.35 & 1.36 ± 1.19 & 1.07 ± 1.10 & 2.66 ± 2.31 \\
			\textcolor{red}{\checkmark} & \textcolor{red}{\checkmark} & \textbf{0.41 ± 0.33} & \textbf{1.29 ± 1.14} & \textbf{0.96 ± 0.80} & \textbf{2.53 ± 2.13} \\
			
			\midrule 
			\bottomrule 
		\end{tabular} 
		\vspace{1em}
		
		\begin{tabular}{cc|cc|cc} 
			\toprule 
			\multicolumn{2}{c|}{\tabincell{c}{(e) Mech\\Ablation}} &
			\multicolumn{2}{c|}{Intersection} & \multicolumn{2}{c}{Roundabout (Transfer)}\\
			
			\midrule 
			\tabincell{c}{TF} &\tabincell{c}{Att}
			&ADE & FDE & ADE & FDE\\
			\midrule 
			\textcolor{red}{×} & \textcolor{red}{×} & \textbf{0.41 ± 0.33} & \textbf{1.29 ± 1.14} & \textbf{0.96 ± 0.80} & \textbf{2.53 ± 2.13} \\
			\checkmark & × & 0.41 ± 0.34 & 1.32 ± 1.16 & 0.97 ± 0.83 & 2.54 ± 2.14 \\
			× & \checkmark & 0.43 ± 0.34 & 1.32 ± 1.13 & 1.10 ± 1.32 & 2.57 ± 2.50 \\
			
			
			\midrule 
			\bottomrule 
		\end{tabular} 
		\caption{The quantitative results for high-level intention identification polices.} 
		\label{tab:encoder_decoder}
% 		\vspace{-2em}
\end{table}

% \begin{table*}[!t]
% 		\label{tab:graph}
% 		\centering
% 		\begin{tabular}{cc|cc|cc|cc|cc|cc} 
% 			\toprule 
% 			\multicolumn{2}{c|}{Speed Ablation} & \multicolumn{2}{c|}{Yaw Ablation} &
% 			\multicolumn{2}{c|}{Representation Ablation} &
% 			\multicolumn{2}{c|}{Mechanism Ablation} &
% 			\multicolumn{2}{c|}{Intersection} & \multicolumn{2}{c}{Roundabout}\\
% 			\midrule 
% 			\tabincell{c}{Input\\Speed} &\tabincell{c}{Output\\Speed} & \tabincell{c}{Input\\Yaw} & \tabincell{c}{Output\\Yaw} & Incremental & Alignment & \tabincell{c}{Teacher\\Forcing} & Attention & ADE & FDE & ADE & FDE\\
% 			\midrule 
% 			× & × & × & × & × & × & × & × & 0.91 ± 0.59 & 1.87 ± 1.48 & 2.96 ± 4.65 & 5.52 ± 7.20 \\
% 			\checkmark & x & × & × & × & × & × & × & 0.71 ± 0.54
%             & 1.53 ± 1.27 & 2.33 ± 3.84 & 4.30 ± 5.44 \\
% 			× & \checkmark & × & × & × & × & × & × & 0.78 ± 0.53 & 1.74 ± 1.41 & 2.51 ± 4.16 & 4.97 ± 6.35 \\
% 			\checkmark & \checkmark & × & × & × & × & × & × & 0.70 ± 0.49 & 1.46 ± 1.26 & 2.40 ± 4.10 & 4.67 ± 6.03 \\
			
% 			\midrule 
% 			\checkmark & × & × & × & × & × & × & × & 0.71 ± 0.54 & 1.53 ± 1.27 & 2.33 ± 3.84 & 4.30 ± 5.44 \\
% 			\checkmark & × & \checkmark & × & × & × & × & × & 0.67 ± 0.46 & 1.45 ± 1.19 & 2.23 ± 3.95 & 4.14 ± 5.19 \\
% 			\checkmark & × & × & \checkmark & × & × & × & × & 0.73 ± 0.50 & 1.59 ± 1.36 & 2.34 ± 3.96 & 4.49 ± 6.46  \\
% 			\checkmark & × & \checkmark & \checkmark & × & × & × & × & 0.67 ± 0.48 & 1.46 ± 1.24 & 2.51 ± 4.60 & 4.77 ± 6.43 \\
			
% 			\midrule 
% 			\checkmark & × & \checkmark & × & \checkmark & × & × & × & 0.48 ± 0.44 & 1.32 ± 1.32 & 1.26 ± 0.95 & 3.04 ± 2.44  \\
% 			\checkmark & × & \checkmark & × & × & \checkmark & × & × & 0.43 ± 0.35 & 1.36 ± 1.19 & 1.07 ± 1.10 & 2.66 ± 2.31 \\
% 			\checkmark & × & \checkmark & × & \checkmark & \checkmark & × & × & 0.41 ± 0.33 & 1.29 ± 1.14 & 0.96 ± 0.80 & 2.53 ± 2.13 \\
			
% 			\midrule 
% 			\checkmark & × & \checkmark & × & \checkmark & \checkmark & \checkmark & × & 0.41 ± 0.34 & 1.32 ± 1.16 & 0.97 ± 0.83 & 2.54 ± 2.14 \\
% 			\checkmark & × & \checkmark & × & \checkmark & \checkmark & × & \checkmark & 0.43 ± 0.34 & 1.32 ± 1.13 & 1.10 ± 1.32 & 2.57 ± 2.50 \\
		
% 			\bottomrule 
% 		\end{tabular} 
% 		\caption{The quantitative results for high-level intention identification polices.} 
% % 		\vspace{-2em}
% \end{table*}


% \begin{table}[!t]
% 		\label{tab:graph}
% 		\centering
% 		\begin{tabular}{cc|cc|cc} 
% 			\toprule 
% 			\multicolumn{2}{c|}{Feature Ablation} & \multicolumn{2}{c|}{Feature Ablation}\\
			
			
% 			\midrule 
% 			\multicolumn{2}{c|}{Speed} &
% 			\multicolumn{2}{c|}{Yaw} &
% 			\multicolumn{2}{c|}{Intersection} & \multicolumn{2}{c}{Roundabout}\\
% 			\midrule 
% 			Incremental & Alignment & ADE & FDE & ADE & FDE\\
% 			\midrule 
% 			× & × & 0.91 ± 0.59 & 1.87 ± 1.48 & 2.96 ± 4.65 & 5.52 ± 7.20 \\
% 			\checkmark & x & 0.71 ± 0.54
%             & 1.53 ± 1.27 & 2.33 ± 3.84 & 4.30 ± 5.44 \\
% 			× & \checkmark & 0.78 ± 0.53 & 1.74 ± 1.41 & 2.51 ± 4.16 & 4.97 ± 6.35 \\
% 			\checkmark & \checkmark & 0.70 ± 0.49 & 1.46 ± 1.26 & 2.40 ± 4.10 & 4.67 ± 6.03 \\
			
% 			\midrule 
% 			\bottomrule 
% 		\end{tabular} 
% 		\caption{The quantitative results for high-level intention identification polices.} 
% % 		\vspace{-2em}
% \end{table}



% \begin{table}[!t]
% 		\label{tab:graph}
% 		\centering
% 		\begin{tabular}{cc|cc|cc|cc} 
% 			\toprule 
% 			\multicolumn{2}{c|}{\tabincell{c}{Speed\\Ablation}} &
% 			\multicolumn{2}{c|}{\tabincell{c}{Yaw\\Ablation}} &
% 			\multicolumn{2}{c|}{Intersection} & \multicolumn{2}{c}{Roundabout}\\
			
% 			\midrule 
% 			\tabincell{c}{In} &\tabincell{c}{Out} &\tabincell{c}{In}
% 			&\tabincell{c}{Out} 
% 			&ADE & FDE & ADE & FDE\\
% 			\midrule 
% 			× & × & × & × & 0.91 ± 0.59 & 1.87 ± 1.48 & 2.96 ± 4.65 & 5.52 ± 7.20 \\
% 			\checkmark & x & × & × & 0.71 ± 0.54
%             & 1.53 ± 1.27 & 2.33 ± 3.84 & 4.30 ± 5.44 \\
% 			× & \checkmark & × & × & 0.78 ± 0.53 & 1.74 ± 1.41 & 2.51 ± 4.16 & 4.97 ± 6.35 \\
% 			\checkmark & \checkmark & × & × & 0.70 ± 0.49 & 1.46 ± 1.26 & 2.40 ± 4.10 & 4.67 ± 6.03 \\
			
% 			\midrule 
% 			\bottomrule 
% 		\end{tabular} 
% 		\caption{The quantitative results for high-level intention identification polices.} 
% % 		\vspace{-2em}
% \end{table}

% \begin{table*}[!t]
% 		\label{tab:graph}
% 		\centering
% 		\begin{tabular}{cc|cc|cc|cc} 
% 			\toprule 
% 			\multicolumn{2}{c|}{Speed Ablation} &
% 			\multicolumn{2}{c|}{Yaw Ablation} &
% 			\multicolumn{2}{c|}{Intersection} & \multicolumn{2}{c}{Roundabout}\\
			
% 			\midrule 
% 			\tabincell{c}{Input\\Speed} &\tabincell{c}{Output\\Speed} &\tabincell{c}{Input\\Yaw}
% 			&\tabincell{c}{Output\\Yaw} 
% 			&ADE & FDE & ADE & FDE\\
% 			\midrule 
% 			× & × & × & × & 0.91 ± 0.59 & 1.87 ± 1.48 & 2.96 ± 4.65 & 5.52 ± 7.20 \\
% 			\checkmark & x & × & × & 0.71 ± 0.54
%             & 1.53 ± 1.27 & 2.33 ± 3.84 & 4.30 ± 5.44 \\
% 			× & \checkmark & × & × & 0.78 ± 0.53 & 1.74 ± 1.41 & 2.51 ± 4.16 & 4.97 ± 6.35 \\
% 			\checkmark & \checkmark & × & × & 0.70 ± 0.49 & 1.46 ± 1.26 & 2.40 ± 4.10 & 4.67 ± 6.03 \\
			
% 			\midrule 
% 			\bottomrule 
% 		\end{tabular} 
% 		\caption{The quantitative results for high-level intention identification polices.} 

% % 		\vspace{-2em}
% \end{table*}

\subsection{Encoder Decoder Network Evaluation}
There are many existing works exploiting encoder decoder architecture for the driving behavior generation\cite{park2018sequence}\cite{tang2019multiple}\cite{zyner2019naturalistic}, but several questions still remain unclear, such as what coodinate should be employed, what features should be considered in EDN, what representation performs better, and whether commonly-used mechanisms in encoder decoder architecture can improve the performance in the driving task. Thus in this section, we experimented the EDN itself without intention signal. Note that, starting from a naive encoder decoder which simply takes in position features and predicts positions, we experimented the factors incrementally. Later experiments inherited the structure verified as the best earlier. We set two metrics, absolute distance error (ADE) and final distance error (FDE).

\subsubsection{Coordinate Study}
Though seemingly intuitive, we first investigated which coordinate should we employ between Frenet and Cartesian coordinate. As shown in Table~\ref{tab:encoder_decoder}(a), we can see the EDN with Frenet coordinate performed 40\% (ADE) and 35\% (FDE) better than EDN with Cartesian coordinate in the intersection scenario. In the zero-transferred roundabout scenario, though both the two methods performed worse, the performance of method with Cartesian coordinate decayed significantly, with ADE higher by 324\%  and FDE higher by 258\% compared to the method with Frenet coordinate.

This is because the Frenet coordinate implicitly incorporate the map information into the model. Compared to running in any directions in the Cartesian coordinate, the vehicles would follow the direction of references paths in the Frenet coordinate, which constrains its behavior in a reasonable range.

\subsubsection{Feature Study}
Second, we explored the effect of features, namely the speed feature and yaw feature. For each feature, we consider two circumstances. The first is to incorporate the feature into the input feature of the encoder to provide more information. The second is to expect the feature as additional desired outputs of the decoder, which could possibly help to stabilize the learning for position feature generation. Thus for each feature, we explored 4 settings in terms of whether or not adding the feature into the input or output, as in Table~\ref{tab:encoder_decoder}(b)(c).

We can see from Table~\ref{tab:encoder_decoder}(b) that, incorporating speed feature in either the input or output could both effectively improve performance in the two scenarios. When simultaneously incorporate it into the input and output, the performance was slightly improved in the intersection scenario and slightly degraded in the roundabout scenario compared the only consider it in the input. Judging from the average performance in two scenarios, we choose only taking speed into the encoder as the approach continued to be used in later experiments.

From Table~\ref{tab:encoder_decoder}(c), we can see that the approach taking the yaw feature into input could slightly benefit the performance, while incorporating it into the output made the performance worse. Such effect decay makes sense as the yaw information is already implicitly hidden in the speed information. Not providing enough information, adding it into the output of decoder indeed made the learning harder. We thus continued to use the method of taking yaw into the input in later experiments.

\subsubsection{Representation Study}
% When viewing the generated behaviors from EDN, we found the generated behavior has always been smooth enough, but we also frequently witnessed obvious behavior shift at the first decoding step due to the incompatibility of context vector and  
There are two techniques about the representation of data for data distributions shaping. The first is to align the positions relative to the vehicle's current position\cite{park2018sequence}. The second is to incrementally generate position difference compared to last step rather than generate absolute position\cite{li2019grip++}.  

From the results in Table~\ref{tab:encoder_decoder}(d), we can see that both the two techniques could significantly benefit the behavior generation, while applying both of them worked the best by improving the ADE by 38\% in the intersection and by 56\% in the roundabout. 

\subsubsection{Mechanism Study}
There are two frequently used mechanism in the encoder decoder architecture: teacher forcing\cite{williams1989learning} and attention\cite{bahdanau2014neural}. Teacher forcing aims at facilitate the learning of complex tasks while the attention is designed to attend to different historic input. 

From the results in Table~\ref{tab:encoder_decoder}(c), we can see neither of the two mechanisms could benefit our model. Considering that the encoder decoder is used as a dynamics approximator, the teacher forcing achieved similar and slightly worse performance because this is a relatively simple task that the EDN itself can learn well enough, while the attention mechanism indeed made the performance worse as the vehicle dynamics is most related to recent state and further state may not be relevant. 

\subsection{Intention Signal Introduction Evaluation}
\label{sec:experiment_intention_signal_intro}
As mentioned in Sec. \ref{sec:intention_signal_intro_method}, we have two intention signals, i.e. goal state and decoding step, which can be introduced into the EDN in several ways, such as appending it into the input or output of the decoder, or embedding it into the hidden state at the first step. For the intention signal, we can additionally choose to introduce it by transforming the origin state of the into state relative to the goal state. 

First, we introduced the ground-truth goal state into the EDN to verify the introduction method. As in Table~\ref{tab:intention}(a), we can see that the Transform method had the best performance and reduced the ADE by 75\% and 56\% in the two scenarios, which represents the most benefit we can get with ground-truth label but is also impossible as there exists unevitable deviations in the goal state generated. Adding goal state into the hidden state also outperformed appending it into the input, while adding it at the output of GRU performed worst.

When consider the generated goal state into EDN, the deviation and variance in the generated goal state would perturb the performance. As in Table~\ref{tab:intention}(b), the effect of several goal state introduction methods were similar, while the appending the goal state into the input feature list performed the best, improving the ADE by 26\% and 10\% in the two scenarios.

After introducing goal state into the input feature, we further investigate introducing the time signal as shown in Table~\ref{tab:intention}(c). Similarly, appending it into the input performed the best, improving the ADE by 26\% and 14\% in the two scenarios compared to no-intention-signal EDN.

In Figure~\ref{fig:Error by Step}, we compared the method with and without intention signal, in terms of the error of each step in the future 30 steps. We can clearly see that as the prediction horizon extends, the prediction error grows exponentially. But the intention signal can effectively suppress the error growth, especially in the long horizon.

\begin{table*}[!t]
		
		\centering
		\begin{tabular}{cc|c|cccc} 
			\toprule 
			\multicolumn{7}{c}{(a) Ground-truth Goal State Introduction}\\
			\midrule 
			Scenario & Measure & No-Label & Transform & Input & Output & Hidden\\
			\midrule 
			\multirow{2}*{Intersection} &  ADE (m) & 0.41 ± 0.11 & \textbf{0.10 ± 0.10} & 0.15 ± 0.13 & 0.17 ± 0.16 & 0.13 ± 0.14\\
			~ & FDE (m) & 1.29 ± 1.30 & \textbf{0.15 ± 0.25} & 0.29 ± 0.40 & 0.38 ± 0.41 & 0.26 ± 0.39\\
			\midrule    
			
			\multirow{2}*{\tabincell{c}{Roundabout\\(Transfer)}} &  ADE (m) & 0.96 ± 0.64 & \textbf{0.42 ± 0.37} & 0.51 ± 0.46 & 0.60 ± 0.54 & 0.48 ± 0.41\\
			~ & FDE (m) & 2.53 ± 4.54 & \textbf{0.72 ± 0.66} & 0.94 ± 0.73 & 1.03 ± 0.74 & 0.84 ± 0.67\\
			\bottomrule 
		\end{tabular} 
		\vspace{1em}
		
		\begin{tabular}{cc|c|cccc} 
			\toprule 
			\multicolumn{7}{c}{(a) Generated Goal State Introduction}\\
			\midrule 
			Scenario & Measure & No-Label & Transform & Input & Output & Hidden\\
			\midrule 
			\multirow{2}*{Intersection} &  ADE (m) & 0.41 ± 0.11 & 0.31 ± 0.25 & \textbf{0.30 ± 0.25} & 0.32 ± 0.25 & 0.31 ± 0.25\\
			~ & FDE (m) & 1.29 ± 1.30 & 0.92 ± 0.85 & 0.89 ± 0.83 & 0.89 ± 0.83 & \textbf{0.89 ± 0.82}\\
			\midrule    
			
			\multirow{2}*{\tabincell{c}{Roundabout\\(Transfer)}} &  ADE (m) & 0.96 ± 0.64 & 0.89 ± 0.56 & \textbf{0.86 ± 0.61} & 0.92 ± 0.75 & 0.87 ± 0.54\\
			~ & FDE (m) & 2.53 ± 4.54 & 2.14 ± 1.44 & \textbf{2.12 ± 1.51} & 2.19 ± 1.69 & 2.22 ± 1.46\\
			\bottomrule 
		\end{tabular} 
		\vspace{1em}
		
		
		\begin{tabular}{cc|c|cccc} 
			\toprule 
			\multicolumn{7}{c}{(a) Time Signal Introduction}\\
			\midrule 
			Scenario & Measure & No-Label & Transform & Input & Output & Hidden\\
			\midrule 
			\multirow{2}*{Intersection} &  ADE (m) & 0.41 ± 0.11 & 0.30 ± 0.25 & \textbf{0.30 ± 0.25} & 0.30 ± 0.25 & 0.30 ± 0.24\\
			~ & FDE (m) & 1.29 ± 1.30 & 0.89 ± 0.83 & 0.88 ± 0.83 & 0.89 ± 0.83 & \textbf{0.88 ± 0.81}\\
			\midrule    
			
			\multirow{2}*{\tabincell{c}{Roundabout\\(Transfer)}} &  ADE (m) & 0.96 ± 0.64 & 0.86 ± 0.61 & \textbf{0.82 ± 0.53} & 0.87 ± 0.59 & 0.84 ± 0.53\\
			~ & FDE (m) & 2.53 ± 4.54 & 2.12 ± 1.51 & \textbf{2.06 ± 1.43} & 2.15 ± 1.51 & 2.11 ± 
			0.23\\
			\bottomrule 
		\end{tabular} 
		\vspace{1em}
		
		
		\caption{The quantitative results for intention signal introduction.} 
		\label{tab:intention}
\end{table*}
\begin{figure*}[t]
    \centering
    \includegraphics[width=0.95\textwidth]{Figures/Error_By_Step.pdf}
    \caption{Prediction error of each step. The prediction error grows exponentially as horizon extends. The intention signal could effectively suppress the error growth, especially in the long term.}
    \label{fig:Error by Step}
    % \vspace{-2em}
\end{figure*}

\subsection{Online Adaptation Evaluation}
\label{exp:adaptation}
As in Figure \ref{fig:adaptation_trajectory}, we designed several metrics to systematically analyze the online adaptation:
\begin{enumerate}
    \item ADE 1: This metric evaluates the performance of the adapted steps on the historic trajectory $Y_{t-\tau, t}$, which basically verifies whether the algorithm is working or not.
    \item ADE 2: This metric evaluates the performance of the adaptation steps on the current trajectory, which aims at verifying how the time lag is influencing the adaptation whether adaptation could benefit current short-term behavior generation.
    \item ADE 3: This metric evaluate the performance of the whole historic trajectory, which implies whether we have get enough information on the behavior pattern.
    \item ADE 4: This metric evaluates the performance of the whole current trajectory, which shows whether the adaptation based on historic information could help current long-term behavior generation.
\end{enumerate}

We run the online adaptation on both the intersection and roundabout scenarios, and collect statistical results of the ADE between ground-truth and generated behavior. We here show how the four metrics evolve with the adaptation step $\tau$.

Figure~\ref{fig:adaptation_analysis}(a) shows the online adaptation results in intersection scenario. In the first two images, we can see as the adaptation step $\tau$ increases, the error of the first $\tau$ step increase for both historic and current trajectory. Also, for the ADE 1, the percentage that online adaptation reduced the error increases along the increasing adaptation step $\tau$ because more information is gained. For the ADE 2, the percentage of error reduction first increases and reached a peak of 20.5\% at 3 adaptation step due to more information, but decreased after that as the behavior gap has happened due to longer time lag. The last two images shows the ADE in the whole historic or current trajectory. For the ADE 3 in the third image, we can see that as $\tau$ increases, the percentage of error reduction also increases with more information. However, for the ADE 4 in the fourth image, we can see that, suppressed by the insufficient information and behavior gap, the improvement is very limited. 

The similar results can be found in the roundabout scenario in Figure~\ref{fig:adaptation_analysis}(b). But in the ADE 2, we can see that more improvement (28\%) is achieved, due to the fact that the model is not trained on the roundabout scenario.

With these analysis, we can find that though the adaptation can not help with the long-term behavior generation, the short-term behavior generation is effectively improved by 20.5\% and  28.7\%. Such improvement in the short-term behavior generation is also important, because it can effectively enhance safety in close-distance interactions.

\begin{figure}[t]
    \centering
    \includegraphics[width=0.5\textwidth]{Figures/Adaptation_Trajectory.pdf}
    \caption{A illustration for adaptation and metric for adaptation analysis. At time step $t$, the model parameters can be adapted by minimizing prediction error of the trajectory in past $\tau$ steps $\textbf{Y}_{t-\tau, t}$. 4 metrics are designed to analyze adaptation performance. ADE 1 can verify how the adaptation works on the source trajectory $\textbf{Y}_{t-\tau, t}$. ADE 2 can verify whether adaptation can benefit short-term prediction in the presence of behavior gap between earlier time and current time. ADE 3 can verify whether we have obtained enough information as we increase the adaptation step $\tau$. ADE 4 verifies whether adaptation can benefit the long-term prediction.}
    \label{fig:adaptation_trajectory}
    \vspace{-2em}
\end{figure}

\begin{figure*}[t]
    \centering
    \includegraphics[width=1\textwidth]{Figures/Adaptation_Analysis.pdf}
    \caption{Adaptation Analysis. In the ADE 1 and ADE 3 in (a)(b), we can see as adaptation step $\tau$ increases, though the prediction error grows, the online adaptation can get more information and improve prediction by a higher percentage. In the ADE 2, we can see as adaptation step $\tau$ increases, the improved percentage first grows higher but then declined, due to the trade-off between more information and behavior gap due to time lag. When $\tau$ is 3, short-term prediction is improved by 20\% and 28\% on the two scenarios respectively. In the ADE 4, we can see online adaptation can barely benefit long-term prediction.}
    \label{fig:adaptation_analysis}
    % \vspace{-2em}
\end{figure*}





\subsection{Overall Evaluation}
\label{sec:overall_evaluation}
\begin{table*}[!t]
		\centering
		\begin{tabular}{ccc|c|cc|cc|c} 
			\toprule 
			& & & & \multicolumn{2}{c|}{EDN Exploration} & \multicolumn{2}{c|}{Intention Integration} & Online Adaptation\\
			\midrule 
			Scenario & Metric & Horizon & Baseline & Feature & Representation & \tabincell{c}{Goal State\\ Signal} & \tabincell{c}{Time\\Signal} & Ours\\
			\midrule 
			\multirow{4}*{Intersection} &  \multirow{2}*{ADE} & 3s  & 0.884 ± 0.594 & 0.629 ± 0.397 & 0.407 ± 0.328 & 0.302 ± 0.251 & 0.305 ± 0.253 & \textbf{0.301 ± 0.250}\\
			~ & ~ & 0.3s & 0.409 ± 0.245 &  0.319 ± 0.224 &  0.027 ± 0.020 &  \textbf{0.021 ± 0.017} &  0.029 ± 0.020 & 0.023 ± 0.014\\
			\cmidrule(r){4-9}    
			~ & \multirow{2}*{FDE} & 3s & 1.850 ± 1.684 & 1.416 ± 1.175 & 1.279 ± 1.130 & 0.890 ± 0.831 & \textbf{0.876 ± 0.835} & 0.877 ± 0.830\\
			~ & ~ & 0.3s & 0.423 ± 0.245 &  0.324 ± 0.229 &  0.040 ± 0.034 &  0.036 ± 0.025 &  0.043 ± 0.032 & \textbf{0.032 ± 0.024}\\
			\midrule 
			
			\multirow{4}*{\tabincell{c}{Roundabout\\(Transfer)}} &  \multirow{2}*{ADE} & 3s & 2.924 ± 4.695 & 2.201 ± 3.999 & 0.941 ± 0.778 & 0.845 ± 0.564 & 0.815 ± 0.526 & \textbf{0.815 ± 0.526}\\
			~ & ~ & 0.3s & 1.572 ± 4.029 & 1.543 ± 3.957 & 0.062 ± 0.071 & 0.060 ± 0.060 & 0.073 ± 0.065 & \textbf{0.052 ± 0.068} \\
			\cmidrule(r){4-9}    
			
			~ &	\multirow{2}*{FDE} & 3s & 5.446 ± 7.157 & 4.123 ± 5.227 & 2.494 ± 2.070 & 2.081 ± 1.440 & 2.038 ± 1.409 & \textbf{2.041 ± 1.409} \\
			~ & ~ & 0.3s & 1.546 ± 3.894 & 1.544 ± 3.944 & 0.088 ± 0.104 & 0.091 ± 0.101 & 0.108 ± 0.107 & \textbf{0.079 ± 0.114}\\
			\bottomrule 
		\end{tabular} 
		\caption{A summary for The quantitative results for comparison with other methods.} 
		\label{tab:overall_comparison}
% 		\vspace{-2em}
\end{table*}
% \begin{table*}[!t]
% 		\label{tab:overall_comparison}
% 		\centering
% 		\begin{tabular}{ccc|c|ccc|cc|c} 
% 			\toprule 
% 			& & & & \multicolumn{3}{c|}{EDN Exploration} & \multicolumn{2}{c|}{Intention Integration} & Online Adaptation\\
% 			\midrule 
% 			Scenario & Metric & Horizon & Baseline & Feature & Representation & Mechanism & \tabincell{c}{Goal State\\ Signal} & \tabincell{c}{Time\\Signal} & Ours\\
% 			\midrule 
% 			\multirow{4}*{Intersection} &  \multirow{2}*{ADE} & 3s  & 0.884 ± 0.594 & 0.629 ± 0.397 & 0.407 ± 0.328 & 0.402 ± 0.338 & 0.302 ± 0.251 & 0.305 ± 0.253 & \textbf{0.301 ± 0.250}\\
% 			~ & ~ & 0.3s & 0.409 ± 0.245 &  0.319 ± 0.224 &  0.027 ± 0.020 &  0.027 ± 0.022 &  0.021 ± 0.017 &  0.029 ± 0.020 & \textbf{0.023 ± 0.014}\\
% 			\cmidrule(r){4-10}    
% 			~ & \multirow{2}*{FDE} & 3s & 1.850 ± 1.684 & 1.416 ± 1.175 & 1.279 ± 1.130 & 1.239 ± 1.113 & 0.890 ± 0.831 & 0.876 ± 0.835 & \textbf{0.877 ± 0.830}\\
% 			~ & ~ & 0.3s & 0.423 ± 0.245 &  0.324 ± 0.229 &  0.040 ± 0.034 &  0.039 ± 0.035 &  0.036 ± 0.025 &  0.043 ± 0.032 & \textbf{0.032 ± 0.024}\\
% 			\midrule 
			
% 			\multirow{4}*{\tabincell{c}{Roundabout\\(Transfer)}} &  \multirow{2}*{ADE} & 3s & 2.924 ± 4.695 & 2.201 ± 3.999 & 0.941 ± 0.778 & 0.919 ± 0.786 & 0.845 ± 0.564 & 0.815 ± 0.526 & \textbf{0.815 ± 0.526}\\
% 			~ & ~ & 0.3s & 1.572 ± 4.029 & 1.543 ± 3.957 & 0.062 ± 0.071 & 0.055 ± 0.055 & 0.060 ± 0.060 & 0.073 ± 0.065 & \textbf{0.052 ± 0.068} \\
% 			\cmidrule(r){4-10}    
			
% 			~ &	\multirow{2}*{FDE} & 3s & 5.446 ± 7.157 & 4.123 ± 5.227 & 2.494 ± 2.070 & 2.422 ± 2.024 & 2.081 ± 1.440 & 2.038 ± 1.409 & \textbf{2.041 ± 1.409} \\
% 			~ & ~ & 0.3s & 1.546 ± 3.894 & 1.544 ± 3.944 & 0.088 ± 0.104 & 0.082 ± 0.094 & 0.091 ± 0.101 & 0.108 ± 0.107 & \textbf{0.079 ± 0.114}\\
% 			\bottomrule 
% 		\end{tabular} 
% 		\caption{The quantitative results for comparison with other methods.} 
% % 		\vspace{-2em}
% \end{table*}
\begin{table*}[!t]
		\centering
		\begin{tabular}{ccc|ccc|cc} 
			\toprule 
			& & & \multicolumn{3}{c|}{Rule-Based Method} & \multicolumn{2}{c}{GNN-Based Method}\\
			\midrule 
			Scenario & Metric & Horizon & IDM & FSM-D & FSM-T & Trajectron++ & Ours\\
			\midrule 
			\multirow{4}*{Intersection} &  \multirow{2}*{ADE} & 3s  & 2.847 ± 1.963 & 3.181 ± 2.403 & 3.372 ± 2.495 & 0.510 ± 0.440 & \textbf{0.301 ± 0.250}\\
			~ & ~ & 0.3s & 0.042 ± 0.014 & 0.051 ± 0.034 & 0.054 ± 0.034 & \textbf{0.009 ± 0.008} & 0.023 ± 0.014\\
			\cmidrule(r){4-8}    
			~ & \multirow{2}*{FDE} & 3s & 7.655 ± 5.536 & 8.709 ± 7.081 & 9.011 ± 7.192 & 1.617 ± 1.517 & \textbf{0.877 ± 0.830}\\
			~ & ~ & 0.3s & 0.091 ± 0.033 & 0.103 ± 0.059 & 0.111 ± 0.059 &  \textbf{0.014 ± 0.013} & 0.032 ± 0.024\\
			\midrule 
			
			\multirow{4}*{\tabincell{c}{Roundabout\\(Transfer)}} &  \multirow{2}*{ADE} & 3s & 5.271 ± 1.950 & 4.637 ± 1.448 & 4.824 ± 1.509 & 1.250 ± 0.849 & \textbf{0.815 ± 0.526}\\
			~ & ~ & 0.3s & 0.126 ± 0.062 & 0.090 ± 0.071 & 0.093 ± 0.070 & \textbf{0.015 ± 0.011} & 0.052 ± 0.068\\
			\cmidrule(r){4-8}    
			
			~ &	\multirow{2}*{FDE} & 3s & 13.891 ± 5.845 & 13.133 ± 4.208 & 13.505 ± 4.407 & 4.063 ± 2.706 & \textbf{2.041 ± 1.409}\\
			~ & ~ & 0.3s & 0.206 ± 0.096 & 0.157 ± 0.105 & 0.162 ± 0.102 & \textbf{0.025 ± 0.020} & 0.079 ± 0.114\\
			\bottomrule 
		\end{tabular} 
		\caption{The quantitative results for comparison with other methods.} 
		\label{tab:SOTA}
% 		\vspace{-2em}
\end{table*}
In this section, we briefly summarize all the experiments our have conducted as a quick take-away for the reader. Table~\ref{tab:overall_comparison} shows distilled results along the development of our method, where we started from a baseline EDN, which takes in the historic position and predicts future trajectory. 

We first explored the EDN itself. By adding features such as speed and yaw, we reduced the ADE in 3 seconds by 28\% and 24\% in the two scenarios. In the representation, we conducted incremental prediction and position alignment. Such design not only effectively reduced the ADE in 3 seconds by 35\% and 57\% in the two scenarios, but also significantly reduced the ADE in 0.3 seconds by 91\% and 95\%. We can consequently conclude that the information of speed and yaw, along with the incremental prediction and position alignment, are vital for the prediction performance in encoder decoder architecture.

We next conducted intention integration. Integrating the goal state signal significantly reduced the ADE in 3 seconds by 25\% and 10\% in the two scenarios. The time signal barely benefit the prediction in the intersection scenario, but it reduced the ADE in 3 seconds of roundabout scenario by 3.5\%. In Figure~\ref{fig:Error by Step}, we also showed the error by step in the future 30 prediction steps. We can clearly see that as the prediction horizon extends, the prediction error grows exponentially. But the intention signal can effectively suppress the error growth, especially in the long horizon. Such result effectively demonstrated the necessity of intention integration.


Finally, the online adaptation is implemented to the model where both goal state and time signal are leveraged. It can be seen that the online adaptation barely improved the ADE in 3 seconds, but the short-term prediction, namely the ADE in 0.3 seconds, is improved by 20\% and 28\% in the intersection and roundabout scenarios. As a result, a conclusion is that though the online adaptation may not be able to help with long-term prediction, but it can help to refine short-term prediction. Such improvement is valuable especially in close-distance prediction, where small prediction shift can make a big difference in terms of safety.

\subsection{Comparison with Other Methods}
In this section, we compare our method with other methods in terms of behavior prediction in different horizon and transferability.

As in Table~\ref{tab:SOTA}, we first consider three rule-based methods. The IDM\cite{treiber2000congested} method basically follows its front car on the same reference path. The FSM-based\cite{zhang2017finite} method will also recognize cars on the other reference paths, and follow the closest front car using the IDM model. When deciding the closest front car, the FSM-D method will compare ego vehicle's distance to the conflict area to that of others, and choose the car with the closest one. The FSM-T method will first calculate each vehicle's time needed to reach the conflict area by assuming they are running in constant speed, and then choose the closest one. We set the parameter for the IDM model identified in urban driving situations\cite{liebner2012driver}.

We can see from Table~\ref{tab:SOTA} that, the rule-based method has not been working well in the prediction task. Several reasons may be possible. First is that intersections and roundabouts are really complicated with intense multi-agent interaction. Simple rules can hardly capture such complex behaviors while systematic rules are hard to manually design. A second reason is that, the parameter in the driving model is hard to specify as it is also scenario-and-individual-specific.

We also implemented trajectron++\cite{salzmann2020trajectron++}, a graph-neural-network-based method. This method takes vehicles as node of a graph and use a graph neural network to conduct relationship reasoning. The map information is integrated by embedding the image of the map. A generative model is then used to predict future actions. Future trajectory is then generated by propagating the vehicle dynamics with the predicted actions.

From Table~\ref{tab:SOTA} we can see that, our method significantly outperformed trajectron++, with ADE in 3 seconds lower by 41\% and 34\% in the intersection and roundabout scenarios respectively. Such results demonstrates that our method's great capability in the long-term prediction, benefiting from our design of semantic hierarchy and transferable representation, and intensive exploration on the algorithms. Nevertheless, trajectron++ performs much better than ours in the short-term prediction. One important reason is that the predicted trajectory of trajectron++ is strictly dynamics-feasible, as it will essentially predict future actions and propagate them through the dynamics. Such results motivate us to include dynamic constrain in our future work.

 


==> 9bio.tex <==

\begin{IEEEbiography}{Michael Shell}
Biography text here.
\end{IEEEbiography}

\begin{IEEEbiographynophoto}{John Doe}
Biography text here.
\end{IEEEbiographynophoto}

\begin{IEEEbiographynophoto}{Jane Doe}
Biography text here.
\end{IEEEbiographynophoto}

